Higher-order Rewriting for Executable Compiler Specifications

In this paper we outline how a simple compiler can be completely specified using higher order rewriting in all stages: parsing, analysis/optimization, and code emission, specifically using the crsx.sf.net system for a small declarative language called "X" inspired by XQuery (for which we are building a production quality compiler in the same way).

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{E. Bonelli (Ed.): 5th International Workshop\\
on Higher-Order Rewriting (HOR'10)\\
EPTCS 49, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.49.3}{10.4204/EPTCS.49.3}}

